Adversarially Robust Models may not Transfer Better: Sufficient Conditions for Domain Transferability from the View of Regularization

Machine learning (ML) robustness and domain generalization are fundamentally correlated: they essentially concern data distribution shifts under adversarial and natural settings, respectively. On one hand, recent studies show that more robust (adversarially trained) models are more generalizable. On the other hand, there is a lack of theoretical understanding of their fundamental connections. In this paper, we explore the relationship between regularization and domain transferability considering different factors such as norm regularization and data augmentations (DA). We propose a general theoretical framework proving that factors involving the model function class regularization are sufficient conditions for relative domain transferability. Our analysis implies that ``robustness" is neither necessary nor sufficient for transferability; rather, regularization is a more fundamental perspective for understanding domain transferability. We then discuss popular DA protocols (including adversarial training) and show when they can be viewed as the function class regularization under certain conditions and therefore improve generalization. We conduct extensive experiments to verify our theoretical findings and show several counterexamples where robustness and generalization are negatively correlated on different datasets.

==> abstract.tex <==

\begin{abstract}
TODO
\end{abstract}

==> adv_train.tex <==

\subsection{Adversarial Training as a Regularizer}
In this section, we show, under certain conditions, why adversarial training may improve domain generalization by viewing adversarial training as a function class regularizer.

We first provide some notation. Let 
\[
\mathcal{F} = \{f_\theta(\cdot) = W^L\phi^{L-1}(W^{L-1}\phi^{L-2}(\dots) +b^{L-1}) + b^L  \}
\]
where $\phi^j$ are activations, $W^j,b^j$ are weight matrix and bias vector, $\theta$ is the collection of parameters (i.e. $\theta = (W^1,b^1,\dots,W^L,b^L)$. For the rest of the article, assume that $\phi^j$ are just ReLUs.


Now fix $x \in \gX$. Define the preactivation as
\begin{align}
 \widetilde{x}^1 &:= W^1x + b^1 \\
    \widetilde{x}^j &:= W^j\phi^{j-1}(\widetilde{x}^{j-1}) + b^j \, , \, j \geq 2
\end{align}

Define the activation pattern $\phi_x := (\phi^1_x,\dots,\phi_x^{L-1}) \in \{0,1\}^m$ such that
for each $j \in [L-1]$
\begin{equation}
   \phi^j_x =  \1(\widetilde{x}^j > 0)
\end{equation}
where $\1$ is applied elementwise.

Now, given an activation pattern $\phi \in \{0,1\}^m$, we define the preimage $X(\phi) := \{ x \in \sR^{d} : \phi_x = \phi\}$

\begin{theorem}\label{th:equiv}
(In the proof of theorem 1 in \citep{roth2020reg})


Let $\epsilon > 0$ s.t. $B^p_\epsilon(x) \subset X(\phi_x)$ where $B^p_\epsilon(x)$ denotes the $l_p$ ball centered at $x$ with radius $\epsilon$. Let $p = \{1,2,\infty\}$ and $q$ be the Holder conjugate of $p$ (i.e. $\frac{1}{p} + \frac{1}{q} = 1$). Then
\begin{align}
    \E_{(x,y)\sim P}[\l(y,f(x)) + \lambda \max_{x^* \in B^p_\epsilon(x)} \norm{f(x) - f(x^*)}_q] = \E_{(x,y)\sim P}[\l(y,f(x)) + \lambda \cdot \epsilon  \max_{v^* \, : \, \norm{v^*}_p \leq 1} \norm{J_{f(x)}v}_q]
\end{align}
\end{theorem}

\textbf{Interpretation:}
This theorem provides an equivalence between the objective functions for adversarial training (left term) and jacobian regularization (right term). 
We give some intuition on the size of $\epsilon$.
Let us first consider a shallow 2 layer network $f(x) = W^2\phi(W^1x+b^1)$. Suppose $W^2 \in \sR^{m_2 \times m_1}$ and $W^1 \in \sR^{m_1 \times d}$. Given a matrix M, let $M_j$ denote the $j$th row of $M$. We study the activation pattern $\phi_x$ which equals
\begin{align}
    \phi_x = (\phi^1_x) = \begin{pmatrix}
    \1 \{ W^1_1x + b^1_1 \} \\
    \vdots \\
    \1 \{ W^1_{m_1}x + b^1_{m_1} \}
    \end{pmatrix}
\end{align}
We wish to compute the largest radius $\epsilon$ such that the activation pattern $\phi_x$ is constant within $B^2_\epsilon(x)$. This is simply the distance from $x$ to the closest hyperplane of the form $H_{W^1_j, b^1_j} = \{x \in \sR^d \, : \, W^1_{j}x + b^1_{j} = 0\}$ where $j = 0,\dots,m_1$ (i.e. $ \epsilon = \min_j \textrm{dist}(x, H_{W^1_j, b^1_j})$). In particular, if $W^1 = I_{d \times d}$ and $b^1 = \bold{0}$, $\epsilon = \min_{j \in d} \lvert x_j \rvert$.  

Furthermore, we note that $\epsilon$ is nondecreasing as a function of the number of layers. However, it has been observed empirically in \citep{roth2020reg} that approximate correspondence holds in a much larger ball.

\bo{this thm 3.4 can be put in appendix and cite and mention in main text}

\begin{definition} (source and target function class)
Let $\gG^S, \gG^T$ be fine tuning function classes for source and target domains, respectively. We define the class of source models as 
\[
 \gH^S = \gG^S \circ \gF = \{g^S \circ f_\theta \, : \, g^S \in \gG^S, f_\theta \in \gF \}  
\]
and the class of target models as
\[
 \gH^T = \gG^T \circ \gF =  \{g^T \circ f_\theta \, : \, g^T \in \gG^T, f_\theta \in \gF \}  
\]
\end{definition}


\begin{definition} (empirical training objective with jacobian regularization)
Let $\lambda, \epsilon > 0$. Take any hypothesis $h_\theta = g^S \circ f_\theta \in \gH^S$. Let $\hat{R}(h_\theta) = \frac{1}{n}\sum_{i=1}^n\ell(h_{\theta}(x_i),y_i)$ denote the empirical risk where $l(\hat{y},y) = \norm{\hat{y}-y}^2$. We define the empirical training objective with jacobian regularization as
\begin{equation}
    \aobj(h_\theta) = \hat{R}(h_\theta)  + \frac{\lambda \cdot \epsilon}{n} \sum_{i=1}^n \norm{J_{h_\theta}(x_i)}_2 
\end{equation}
\end{definition}

\begin{theorem}\label{th:adv}
Fix regularization strength $\lambda > 0$.
Define 
\[
\mathcal{F}^{A}_\lambda = \{f^A_\theta \in \mathcal{F} : \exists g^S \in \gG^S \, \mathrm{s.t.} \,~ \aobj(g^S \circ f^A_\theta) \leq \aobj(\bold{0}) \}
\]
where $\bm{0}$ denotes the zero function (i.e. the class of feature extractors that outperform the zero function). Suppose $(x,y) \in \gX \times \gY$ is bounded such that  $\max{(\norm{x}_{\infty} ,\norm{y}_{2} )} \leq R$. Fix $\delta > 0$.
Suppose we additionally restrict our fine tuning class models to linear models where 
\[
G^S = \{ W \, : \, W \in \R^{d \times n}, n \geq 1, \min_j \norm{W_j}_{2} \geq  \delta \}
\]
(where $W_j$ is the jth column of $W$) and 
\[
G^T = \{ W \, : \, W \in \R^{d \times n}, n \geq 1 \}
\]
(Here we are abusing notation to let $g^S \in G^S$ to denote the last linear layer as well as the fine tuning function).

Then for $0 \leq \lambda_1 < \lambda_2$
 \begin{equation}
     \gF^A_{\lambda_2} \subsetneq \gF^A_{\lambda_1}  \subsetneq \gF
 \end{equation}
 (where $\subsetneq$ denotes proper subset). In particular, if $H^{A,T}_\lambda = \gG^T \circ \gF^A_\lambda$, we have
  \begin{equation}
     \gH^{A,T}_{\lambda_2} \subsetneq \gH^{A,T}_{\lambda_1} \subsetneq \gH^T
 \end{equation}
\end{theorem}


\textbf{Interpretation:} 




At the high level, this theorem captures the idea that minimizing the empirical risk with jacobian regularization puts a constraint on the set of feature extractors. In particular, $\gF^A_{\lambda_1}$ represents the potential class of feature extractors we select after training with jacobian regularization. Therefore, the class of fine tuned models $H^{A,T}_{\lambda_1}$ with feature extractors trained with jacobian regularization for the target domain is smaller than the class of fine tuned models $\gH$ with feature extractors trained without any regularization. Furthermore, we show that the space of feature extractors shrinks as we increase the regularization stength $\lambda$. Since we showed in section 3.3 that smaller function classes have smaller $d_{\gF_A}$, this theorem shows that jacobian regularization reduces  $d_{\gF_A}$. To connect back to adversarial training, if $\epsilon$ satisfies the hypothesis in theorem $\ref{th:equiv}$, we have that 
\begin{align}
    \E_{(x,y)\sim P}[\l(y,f(x)) + \lambda \max_{x^* \in B^p_\epsilon(x)} \norm{f(x) - f(x^*)}_q] = \E_{(x,y)\sim P}[\l(y,f(x)) + \lambda \cdot \epsilon  \max_{v^* \, : \, \norm{v^*}_p \leq 1} \norm{J_{f(x)}v}_q]
\end{align}
Therefore, minimizing the training objective with jacobian regularization is equivalent to minimizing the adversarial training objective. Using this connection, this theorem essentially shows that, given sufficient number of samples, adversarial training reduces the class of feature extractors which in turn reduces $d_{\gF_A}$.

Finally, we comment on the assumption that $\norm{g^S} > \delta$. Since $\delta > 0$ is arbitrary, we can make it as small as we like and thus we are essentially excluding the $\bold{0}$ last layer which is hardly a constraint on the function class. This assumption is necessary as we are considering regularization on the whole model $g \circ f$ as opposed to regularization on just the feature extractor. Thus, this assumption prevents the scenario where only the last linear layer is regularized.

\begin{proof}
We first show that if $0 \leq \lambda_1 < \lambda_2$, we have that
 \begin{equation}
     \gF^A_{\lambda_2} \subsetneq \gF^A_{\lambda_1}  \subsetneq \gF
 \end{equation}
 
 We first prove the following lemma
 \begin{lemma}\label{lem:eq}
 Suppose the conditions of theorem $\ref{th:adv}$ are satisfied. Suppose additionally we have that $\overline{y} := \frac{1}{n} \sum_{i=1}^d y_i \neq 0$ (note this occurs with probability 1 if marginal distribution  over $\gY$ is continuous). Then for every $\lambda \geq 0$, there exists a function $f_{\theta} \in \gF^A_{\lambda}$ and a fine tuning layer $g^* \in \gG^S$ such that 
 \[
 \aobj(g^* \circ f_\theta) = \inf_{g \in G^S} \aobj(g \circ f_\theta) = \aobj(\bold{0})
 \]
 
Choose another $\lambda' \geq 0$ (can equal $\lambda$). Then there exists a $g^{*}' \in \gG^S$ be the fine tuning layer  such that $\inf_{g \in \gG^S} \aobj[\lambda'](g \circ f_\theta) =  \aobj[\lambda'](g^*' \circ f_\theta) $ and
 \[
\frac{1}{n} \sum_{i=1}^n\norm{J_{g^*' \circ f_\theta}(x_i)}_2 > 0 
 \]
 \end{lemma}
 
 
 \begin{proof}
 
 Fix $\alpha \geq 0$ and $c > \alpha \cdot R$. Set biases
 \begin{align}
     b^1 = \begin{pmatrix}
     c \\
     0\\
     \vdots \\
     0
     \end{pmatrix}
\, b^j = \bold{0}
 \, , \, j \geq 2
 \end{align}
 and weights
  \begin{align}
     W^1 =\begin{pmatrix}
    \alpha & 0 & \dots & 0 \\
    0 & 0 & \dots & 0 \\
    \vdots & \vdots & \vdots & \vdots \\
    0 & \dots & \dots & 0 \\
    \end{pmatrix}
\, W^j =\begin{pmatrix}
    1 & 0 & \dots & 0 \\
    0 & 0 & \dots & 0 \\
    \vdots & \vdots & \vdots & \vdots \\
    0 & \dots & \dots & 0 \\
    \end{pmatrix}
 \, , \, j \geq 2
 \end{align}
 
 Define $x_{i,j}$ be the $j$th entry of the data point $x_i$. Define 
 \begin{align}
     \alpha_i &:=  \alpha \cdot x_{i,1}  \\
     \overline{\alpha} &:= \frac{1}{n} \sum_{i=1}^d\alpha_i \\
    \overline{y} &:= \frac{1}{n} \sum_{i=1}^d y_i
 \end{align}
 
 Now we observe that for a fixed $\lambda \geq 0$ and any $g \in \gG^S$, we have that 
 \begin{align}
      \aobj(g\circ f_{\theta}) &= \hat{R}(g \circ f_{\theta}) + \lambda \cdot \epsilon \frac{1}{n} \sum_{i=1}^n\norm{J_{g \circ f_{\theta}}(x_i)}_2 \\
       &= \frac{1}{n}\sum_{i=1}^n \norm{(\alpha x_{i,1} + c)\begin{pmatrix}
       g_{11} \\
       \vdots \\
       g_{d1}
       \end{pmatrix} - y_i}^2_2 + \lambda \cdot \epsilon \frac{1}{n} \sum_{i=1}^n\norm{g \begin{pmatrix}
    \alpha & 0 & \dots & 0 \\
    0 & 0 & \dots & 0 \\
    \vdots & \vdots & \vdots & \vdots \\
    0 & \dots & \dots & 0 \\
    \end{pmatrix}}_2 \\
     &= \frac{1}{n}\sum_{i=1}^n  \norm{( \alpha_i + c) g_1 - y_i}^2_2 + \lambda \cdot \epsilon \frac{1}{n} \sum_{i=1}^n \alpha \norm{g_1}_2 \\
      &= \frac{1}{n}\sum_{i=1}^n  \norm{( \alpha_i + c) g_1 - y_i}^2_2 + \lambda \cdot \epsilon \alpha \norm{g_1}_2 
 \end{align}
 Therefore, 
 \begin{align}
     \inf_{g \in \gG^S}   \aobj(g\circ f_{\theta})
 \end{align}
 is equivalent to solving
  \begin{align}
     \inf_{w \in \R^d \, : \, \norm{w}_2 \geq \delta }  \frac{1}{n}\sum_{i=1}^n  \norm{( \alpha_i + c) w - y_i}^2_2 + \lambda \cdot \epsilon \alpha \norm{w}_2 \label{minprob}
 \end{align}
 Utilizing lagrange multipliers, we find the minimizer is  
 \begin{align}
     w = \delta \cdot \frac{\overline{y}}{\norm{\overline{y}}} \label{minimizer}
 \end{align}
 when $c \geq \frac{\norm{\overline{y}}_2}{\delta}$. 
 
 Now consider the function 
 \[
 S(c,\alpha) =  \frac{1}{n}\sum_{i=1}^n  \norm{( \alpha \cdot x_{i,1} + c) g_1 - y_i}^2_2 + \lambda \cdot \epsilon \alpha \norm{g_1}_2 
 \]
 Note that this function is continuous with respect to the input $(c,\alpha)$. Now fix $\alpha = 0, c = \frac{\norm{\overline{y}}_2}{\delta}$. Set $w = \delta \cdot \frac{\overline{y}}{\norm{\overline{y}}}$. Then we have that 
\begin{align}
    S(\frac{\norm{\overline{y}}_2}{\delta},0) =  \frac{1}{n}\sum_{i=1}^n  \norm{\overline{y} - y_i}^2_2 < \frac{1}{n}\sum_{i=1}^n  \norm{y_i}^2_2 &= \aobj(\bold{0})
\end{align}
The inequality comes from the fact that we assumed $\overline{y} \neq 0$ and noting that $\overline{y}$ is the minimizer of the function $p(z) = \frac{1}{n}\norm{z - y_i}^2_2 $. Continuity of $S$ ensures that there exists $\alpha_0 > 0$ such that 
\begin{align}
    S(\frac{\norm{\overline{y}}_2}{\delta},\alpha_0) < \frac{1}{n}\sum_{i=1}^n  \norm{y_i}^2_2 &= \aobj(\bold{0})
\end{align}
 Now consider $U(t) = S((1+t)\frac{\norm{\overline{y}}_2}{\delta},(1+t)\alpha_0 )$ for $t \geq 0$. Note that $U$ is continuous with respect to $t$. Furthermore, we note that $t \rightarrow \infty$ implies $U(t) \rightarrow \infty$ which implies there exists some time $t = T_f$ such that $U(T_f) > \aobj(\bold{0})$. Therefore, by the intermediate value theorem, there exists a time $t = T$ such that $U(T) =  \aobj(\bold{0})$. Finally, set $c = (T+1)\frac{\norm{\overline{y}}_2}{\delta}$, $\alpha = (T+1)\alpha_0$, and $g^*$ as the matrix where $g^*_1 = \delta \cdot \frac{\overline{y}}{\norm{\overline{y}}}$ and $\bold{0}$ for the other columns. By equation $\ref{minprob}$ and equation $\ref{minimizer}$  we have
 \begin{align}
      \aobj(g^* \circ f_{\theta}) = \inf_{g \in \gG^S}   \aobj(g\circ f_{\theta}) = U(T) = \aobj(\bold{0}) 
 \end{align}
 Furthermore, if we choose another $\lambda' \geq 0$, since $c = (T+1)\frac{\norm{\overline{y}}_2}{\delta} > \frac{\norm{\overline{y}}_2}{\delta}$ by equation $\ref{minimizer}$, we have that 
  \begin{align}
      \aobj[\lambda'](g^*' \circ f_{\theta}) = \inf_{g \in \gG^S}   \aobj[\lambda'](g\circ f_{\theta}) 
 \end{align}
 and 
   \begin{align}
    \frac{1}{n} \sum_{i=1}^n\norm{J_{g^*' \circ f_\theta}(x_i)}_2 = \alpha \norm{g^*'}_2 = \alpha \delta 
 \end{align}
 which is nonzero as $\delta > 0$ and $\alpha = (T+1)\alpha_0 > 0$.
 
 \end{proof}
 
 
Clearly, we have $\gF^A_{\lambda_2} \subset \gF^A_{\lambda_1}$. If we can show that $f_{\theta_1} \not\in \gF^A_{\lambda_2}$ then we have 
 $\gF^A_{\lambda_2} \subsetneq \gF^A_{\lambda_1}$. 
 
 Using lemma $\ref{lem:eq}$ we can find $f_{\theta_1} \in \gF^A_{\lambda_1}$ such that 
 \[
 \inf_{g \in G^S} \aobj[\lambda_1](g \circ f_{\theta_1}) = \aobj[\lambda_1](\bold{0})
 \]
 In addition lemma $\ref{lem:eq}$ guarantees  minimizers $g^*_1$ and $g^*_2$ such that 
 \begin{align}
     \aobj[\lambda_1](g^*_1 \circ f_{\theta_1}) &= \inf_{g \in G^S} \aobj[\lambda_1](g \circ f_{\theta_1}) \, \textrm{and} \, \frac{1}{n} \sum_{i=1}^n\norm{J_{g^*_1 \circ f_\theta}(x_i)}_2 > 0  \\
      \aobj[\lambda_2](g^*_2 \circ f_{\theta_1}) &= \inf_{g \in G^S} \aobj[\lambda_2](g \circ f_{\theta_1}) \, \textrm{and} \, \frac{1}{n} \sum_{i=1}^n\norm{J_{g^*_2 \circ f_{\theta_1}}(x_i)}_2 > 0  
 \end{align}
 Thus, we have that
 \begin{align}
     \aobj[\lambda_1](g^*_2 \circ f_{\theta_1}) &= \hat{R}(g^*_2 \circ f_{\theta_1}) + \lambda_2 \cdot \epsilon \frac{1}{n} \sum_{i=1}^n\norm{J_{g^*_2 \circ f_{\theta_1}}(x_i)}_2 \\
     &> \hat{R}(g^*_2  \circ f_{\theta_1}) + \lambda_1 \cdot \epsilon \frac{1}{n} \sum_{i=1}^n\norm{J_{g^*_2 \circ f_{\theta_1}}(x_i)}_2  &\textrm{since}~ \lambda_2 > \lambda_1\\
     &\geq \hat{R}(g^*_1  \circ f_{\theta_1}) + \lambda_1 \cdot \epsilon \frac{1}{n} \sum_{i=1}^n\norm{J_{g^*_1 \circ f_{\theta_1}}(x_i)}_2  &\textrm{def of }~ g^*_1\\
     &= \aobj[\lambda_1](\bold{0}) &\textrm{lemma $\ref{lem:eq}$}\\
 \end{align}
 
Thus $f_{\theta_1} \not\in \gF^A_{\lambda_2}$ which implies $\gF^A_{\lambda_2} \subsetneq \gF^A_{\lambda_1}$. It remains to show for $\lambda_1 \geq 0$, we have that $\gF^A_{\lambda_1}  \subsetneq \gF$. 


Consider any $g \in \gG^S$. For $j \in [L]$, define $W^j$ as the weight matrix where $W^j = I_{d \times d}$ (identity matrix) for $j \in [L-1]$ and let the final weight $W^L = B\cdot I_{d \times d}$ for some constant $B > 0$. Set the bias vectors $b^j = \bold{0}$ for $j \geq 2$. Let the first bias equal $b^1 = R \cdot \1$ where $\1$ is the vector of all 1's and $R$ is the upper bound such that $\norm{x}_\infty \leq R$. Set $\theta = (W^1,b^1,\dots,W^L,b^L)$ and let $h_\theta = g \circ f_\theta$

We compute 
\begin{align}
    \aobj[\lambda_1](h _{\theta}) &= \hat{R}(h_\theta) + \lambda_1 \cdot \epsilon \frac{1}{n} \sum_{i=1}^n\norm{J_{h_{\theta}}(x_i)}_2 \\
    &= \frac{1}{n} \sum_{i=1}^n \norm{B(x_i+R\1) - y_i}^2  + \frac{1}{n} \sum_{i=1}^n\norm{J_{h_{\theta}}(x_i)}_2  \\
    &= \frac{1}{n} \sum_{i=1}^n \norm{B(x_i+R\1) - y_i}^2 +   B \norm{g}_2  \\
    &\geq \frac{1}{n} \sum_{i=1}^n \norm{B(x_i+R\1) - y_i}^2 +   B \delta  
\end{align}

We note that sending $B \rightarrow \infty$ we get $\aobj[\lambda_1](h _{\theta}) \rightarrow \infty$ which implies that there exists a $B = B'$ such that $\aobj[\lambda_1](h _{\theta}) > \aobj[\lambda_1](\bold{0})$. Setting $B = B'$ implies $f_\theta \not\in \gF^A_{\lambda_1}$. 


















\end{proof}
